One-dimensional Quantum Gravity and the Schwarzian theory

We develop a model of one-dimensional (Conformal) Quantum Gravity. By discussing the connection between Goldstone and Gauge theories, we establish that this model effectively computes the partition function of the Schwarzian theory where the $\textrm{SL}(2,\mathbb{R})$ symmetry is realized on the base space. The computation is straightforward, involves a local quantum measure and does not rely on localization arguments. Non-localities in the model are exclusively related to the value of fixed gauge invariant moduli. Furthermore, we study the properties of these models when all degrees of freedom are allowed to fluctuate. We discuss the UV finiteness properties of these systems and the emergence of a Planck's length.

==> preamble.tex <==


% bibliography
\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{arXiv:#1}}

% \usepackage[style=numeric-comp, eprint=true, natbib, maxbibnames=10, giveninits=true, sorting=none, useprefix=true]{biblatex}
% \DeclareFieldFormat*{title}{\emph{#1}}
% \DeclareFieldFormat{pages}{#1}% no prefix for the `pages` field in the bibliography
% \DeclareFieldFormat{labelalpha}{\textsc{#1}}
% \renewcommand*{\mkbibnamefamily}[1]{\textsc{#1}}
% \renewcommand*{\mkbibnameprefix}[1]{\textsc{#1}}
% \renewcommand*{\mkbibnamegiven}[1]{\textsc{#1}}
\usepackage{cite}



% Commands
\RequirePackage{mdframed}
\newenvironment{claim}{\begin{mdframed}[linecolor=black!10, backgroundcolor=black!10]\noindent\ignorespaces}{\end{mdframed}}

\RequirePackage[thicklines]{cancel}
\newcommand\ccancel[2][maorange]{\renewcommand\CancelColor{\color{#1!60}}\cancel{#2}}
\newcommand\ccancelto[2][maorange]{\renewcommand\CancelColor{\color{#1!60}}\cancelto{#2}}




\newcommand{\nn}{\nonumber \\}
\newcommand{\et}{\&\ }

% =-like symbols
\let\coloneqq\relax
\let\eqqcolon\relax
\makeatletter
\newcommand*{\coloneqq}{\mathrel{\rlap{\raisebox{0.3ex}{$\m@th\cdot$}}\raisebox{-0.3ex}{$\m@th\cdot$}}=}
\newcommand*{\eqqcolon}{\mathrel{=\llap{\raisebox{0.3ex}{$\m@th\cdot$}}\llap{\raisebox{-0.3ex}{$\m@th\cdot$}}}}
\makeatother
\newcommand{\roteqq}{\text{\rotatebox{90}{$=$}}}
\newcommand{\rotequiv}{\text{\rotatebox{90}{$\equiv$}}}
\newcommand{\rotcoloneqq}{\text{\rotatebox{90}{$\coloneqq$}}}
\newcommand{\roteqqcolon}{\text{\rotatebox{90}{$\eqqcolon$}}}
\newcommand{\demeqq}{\overset{!}{=}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}

% Physics
\newcommand{\hilb}{\cH} % Hilbert space
\DeclareDocumentCommand\parti{}{\subbraces{\mathcal{Z}}} % partition function
\newcommand{\anom}[1]{\parti_{\SPT}\qty[#1]} % anomaly function
\newcommand{\pd}{\partial} % partial derivative
\let\f\relax
\newcommand{\f}[2]{{#1}_{\qty[#2]}} % p-form
\newcommand{\g}[2]{#1^{\qty[#2]}} % p-form group
\newcommand{\inv}[1]{{{#1}^{-1}}}
\newcommand{\adj}[1]{{{#1}^{\dagger}}}
\newcommand{\trans}[1]{{{#1}^{\top}}}
\newcommand{\conj}[1]{{#1^*}}
\renewcommand{\b}[1]{{\overline{#1}}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\Half}{\frac{1}{2}}
\newcommand{\sd}[1]{\qty[#1]} % scaling dimension
\newcommand{\po}{\text{\scalebox{1.3}{$\wp$}}} % Path ordering
\newcommand{\tord}{\mathrm{T}} % time ordering 
\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\I}{\mathrm{I}} % identity

% maths
% \newcommand{\Hom}[1]{\mathrm{Hom}\qty(#1)}
\newcommand{\hg}[1][1]{\uppi_{#1}} % homotopy group
\newcommand{\Rep}{\text{Rep}} % representation
\newcommand{\suchthat}{\;\middle|\;}
\newcommand\ccolon{\text{\scalebox{1.2}{\raisebox{-.2ex}{\stackanchor[.28ex]{.}{.}}}}}
\newcommand{\no}[1]{\; \ccolon {#1} \ccolon \;} % normal ordering

\let\cedille\c
\renewcommand{\c}{\mathbin{\cup}} %cup product [requires \usepackage{amssymb}]
\def\cc#1{\mathbin{\upperset{#1}{\cup}}} %Steenrod higher cup product [requiress \usepackage{amssymb}]


\renewcommand{\vdot}{\cdot} % avoid some physics package nonsense
\renewcommand{\vnabla}{\nabla} % avoid some physics package nonsense
\newcommand{\w}{\mathbin{\scalebox{0.8}{$\wedge$}}}
\newcommand{\ex}[1]{\mathrm{e}^{#1}} % exponential
\renewcommand{\i}{\mathrm{i}} % imaginary unit
\newcommand{\h}{\scalebox{0.9}{$\star$}} %Hodge star

\let\C\undefined
\let\U\undefined
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zx}{\mathbb{Z}^{\times}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\CP}{\mathbb{CP}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\B}{\mathrm{B}} %classifying space
\newcommand{\set}[1]{\qty{#1}}
\newcommand{\sset}[1]{\qty{1,2,\ldots,#1}}
\newcommand{\ssset}{\qty{1,2,\ldots}}
\newcommand{\eqv}{\Longleftrightarrow}

\newcommand{\U}{\mathrm{U}}
\newcommand{\SU}{\mathrm{SU}}
\renewcommand{\O}{\mathrm{O}}
\newcommand{\SO}{\mathrm{SO}}
\renewcommand{\P}{\mathrm{P}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\alg}[1]{\mathfrak{#1}}
\renewcommand{\sl}{\alg{sl}}
\newcommand{\su}{\alg{su}}
\newcommand{\so}{\alg{so}}
\renewcommand{\sp}{\alg{sp}}
\renewcommand{\u}{\alg{u}}

\newcommand{\ct}{\mathrm{T}^*}
\newcommand{\tb}{\mathrm{T}}
\renewcommand{\L}{\mathrm{L}}
\DeclareMathOperator{\Stab}{Stab}
\newcommand{\id}{\mathsf{id}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\gauge}{/\!\!/}

\renewcommand{\H}{\mathrm{H}} %cohomology

\newcommand{\lint}{\int\limits}
\renewcommand{\t}[1]{{\text{#1}}}
\newcommand{\nspace}[1][1]{\kern-#1em}
\newcommand{\blob}{\bullet}
\newcommand{\oblob}{\circ}
\newcommand{\longto}{\longrightarrow}
\newcommand{\xto}[1]{\overset{#1}{\to}}
\renewcommand{\xmapsto}[1]{\overset{#1}{\mapsto}}
\renewcommand{\mod}{\ \text{mod}\ }
\renewcommand{\emptyset}{\varnothing}

\renewcommand{\ip}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\pip}[2]{\left\llangle#1,#2\right\rrangle}


\RequirePackage{interval}
\intervalconfig{soft open fences}
\newcommand{\ropen}[2]{\interval[open right]{#1}{#2}}
\newcommand{\lopen}[2]{\interval[open left]{#1}{#2}}
\newcommand{\open}[2]{\interval[open]{#1}{#2}}
\newcommand{\closed}[2]{\interval{#1}{#2}}

% \cal, \frak, etc.
% \DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n} % resets mathcal if needed
\def \cA {\mathcal{A}}
\def \cB {\mathcal{B}}
\def \cC {\mathcal{C}}
\def \cD {\mathcal{D}}
\def \cE {\mathcal{E}}
\def \cF {\mathcal{F}}
\def \cG {\mathcal{G}}
\def \cH {\mathcal{H}}
\def \cI {\mathcal{I}}
\def \cJ {\mathcal{J}}
\def \cK {\mathcal{K}}
\def \cL {\mathcal{L}}
\def \cM {\mathcal{M}}
\def \cN {\mathcal{N}}
\def \cO {\mathcal{O}}
\def \cP {\mathcal{P}}
\def \cQ {\mathcal{Q}}
\def \cR {\mathcal{R}}
\def \cS {\mathcal{S}}
\def \cT {\mathcal{T}}
\def \cU {\mathcal{U}}
\def \cV {\mathcal{V}}
\def \cW {\mathcal{W}}
\def \cX {\mathcal{X}}
\def \cY {\mathcal{Y}}
\def \cZ {\mathcal{Z}}

\def \sA {\mathscr{A}}
\def \sB {\mathscr{B}}
\def \sC {\mathscr{C}}
\def \sD {\mathscr{D}}
\def \sE {\mathscr{E}}
\def \sF {\mathscr{F}}
\def \sG {\mathscr{G}}
\def \sH {\mathscr{H}}
\def \sI {\mathscr{I}}
\def \sJ {\mathscr{J}}
\def \sK {\mathscr{K}}
\def \sL {\mathscr{L}}
\def \sM {\mathscr{M}}
\def \sN {\mathscr{N}}
\def \sO {\mathscr{O}}
\def \sP {\mathscr{P}}
\def \sQ {\mathscr{Q}}
\def \sR {\mathscr{R}}
\def \sS {\mathscr{S}}
\def \sT {\mathscr{T}}
\def \sU {\mathscr{U}}
\def \sV {\mathscr{V}}
\def \sW {\mathscr{W}}
\def \sX {\mathscr{X}}
\def \sY {\mathscr{Y}}
\def \sZ {\mathscr{Z}}

% \usepackage{calc}


% Tweaking the {physics} package | needs {xparse}

\DeclareDocumentCommand\subbraces{ m o d() }
{
    \IfNoValueTF{#3}
    {#1 \IfNoValueTF{#2}{}{[#2]}}
    {#1 \IfNoValueTF{#2}{}{_{\text{#2}}} \argopen[#3\argclose]}
}

\def\fdiffd{\mathrm{D}}
\DeclareDocumentCommand\fdifferential{ o g d() }{ % Functional Differential 'D'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
        {\fdiffd\IfNoValueTF{#1}{}{^{#1}}}
        {\mathinner{\fdiffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
    }
    {\mathinner{\fdiffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
}
\DeclareDocumentCommand\DD{}{\fdifferential}

\DeclareDocumentCommand\variation{ o g d() }{ % Functional variation
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(F(g))
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
        {\updelta \IfNoValueTF{#1}{}{^{#1}}}
        {\mathinner{\updelta \IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
    }
    {\mathinner{\updelta \IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
}
\DeclareDocumentCommand\var{}{\variation} % Shorthand for \variation


\DeclareDocumentCommand\detp{}{\opbraces{\determinant{}'}}

\DeclareDocumentCommand\act{}{\subbraces{S}}


\DeclareMathOperator{\pfaffian}{pf}
\DeclareDocumentCommand\pf{}{\opbraces{\pfaffian}}

\DeclareMathOperator{\diffeomorphism}{diff}
\DeclareDocumentCommand\diff{}{\opbraces{\diffeomorphism}}

\DeclareMathOperator{\volume}{vol}
\DeclareDocumentCommand\vol{}{\opbraces{\volume}}

\DeclareMathOperator{\rangeof}{range}
\DeclareDocumentCommand\range{}{\opbraces{\rangeof}}

\DeclareMathOperator{\kernel}{ker}
\DeclareDocumentCommand\ker{}{\opbraces{\kernel}}

% \DeclareMathOperator{\schwarzian}{Sch}
% \DeclareDocumentCommand\Sch{}{\trigbraces{\schwarzian}}

\DeclareMathOperator{\faddeevpopov}{\blacktriangle}
\DeclareDocumentCommand\fpdet{}{\opbraces{\faddeevpopov}}

\DeclareMathOperator{\homomorphism}{Hom}
\DeclareDocumentCommand\Hom{}{\opbraces{\homomorphism}}

\renewcommand{\ordersymbol}{\mathrm{O}}

\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\makeatother
